Overlapping Domain Decomposition Preconditioner for Integral Equations

The discretization of certain integral equations, e.g., the first-kind Fredholm equation of Laplace's equation, leads to symmetric positive-definite linear systems, where the coefficient matrix is dense and often ill-conditioned. We introduce a new preconditioner based on a novel overlapping domain decomposition that can be combined efficiently with fast direct solvers. Empirically, we observe that the condition number of the preconditioned system is $O(1)$, independent of the problem size. Our domain decomposition is designed so that we can construct approximate factorizations of the subproblems efficiently. In particular, we apply the recursive skeletonization algorithm to subproblems associated with every subdomain. We present numerical results on problem sizes up to $16\,384^2$ in 2D and $256^3$ in 3D, which were solved in less than 16 hours and three hours, respectively, on an Intel Xeon Platinum 8280M.

==> bak.tex <==



\begin{table}
    \centering \small 
    \caption{\em Maximum and minimum eigenvalues of the preconditioned matrix in 1D. The problem domain $\Omega = [0,1]$ is partitioned into two subdomains.}
    \label{t:jacobi_1d}
    %\begin{subtable}[h]{\textwidth}
    \centering
    \begin{tabular}{cc|ccc} 
    \toprule
      $N$    &  D     & $\lambda_{\max}$  & $\lambda_{\min}$ & $\lambda_{\max}+\lambda_{\min}$  \\ \midrule 
      32     & 2      & 1.7060     & 0.2940  & 2.0000   \\
      64     & 2     & 1.7577     & 0.2423  & 2.0000   \\
      128   & 2     & 1.7968  & 0.2032  & 2.0000   \\
      256   & 2     & 1.8271  & 0.1729 & 2.0000    \\
    \bottomrule
    \end{tabular}
    %\caption{Jacobi preconditioner}
    %\end{subtable}
%    % 2nd 
%    \begin{subtable}[h]{\textwidth}
%    \centering
%    \begin{tabular}{cc|ccc} 
%    \toprule
%      $N$    &  D     & $\lambda_{\max}$  & $\lambda_{\min}$ & $\lambda_{\max}+\lambda_{\min}$  \\ \midrule 
%      32     & 2      & 1.1816     & 0.8184  & 2.0000   \\
%      64     & 2     & 1.2600     & 0.7400  & 2.0000   \\
%      128   & 2     & 1.3341  & 0.6659  & 2.0000   \\
%      256   & 2     & 1.4021  & 0.5979 & 2.0000    \\
%    \bottomrule
%    \end{tabular}
%    \caption{Schwarz preconditioner}
%    \label{t:schwarz_1d}
%    \end{subtable}
\end{table}




\subsection{Schwarz preconditioner} \label{result:schwarz}

The first numerical experiment compares the Jacobi preconditioner with the Schwarz preconditioner on the number of PCG iterations. As \cref{t:pcg} shows, the Jacobi preconditioner led to significantly more iterations, especially for solving  problems in 2D. Empirically, the iteration number increased as $\bigO(M^{1/d})$ with both preconditioners (when $M=\bigO(N)$), although that with the Schwarz preconditioner increased slowly when the problem size was small. 


\begin{table}
    \centering \small 
    \caption{\em PCG iterations $n_{it}$ with the Jacobi preconditioner and the Schwarz preconditioner in 2D (left) and in 3D (right), respectively. All runs target \num{1e-12} relative residual tolerance in PCG. }
    \label{t:pcg}
    \begin{tabular}{cccc} 
    \toprule
      $N$   &  $M$ & Jacobi & Schwarz \\ \midrule 
      $16^2$ & $2^2$ & 34 & 18  \\
      $32^2$ & $4^2$ & 87 & 28  \\
      $64^2$ & $8^2$ & 155 &  33  \\
      $128^2$ & $16^2$ & 245 &  45  \\
    \bottomrule
    \end{tabular}
    \hspace{1cm}
    \begin{tabular}{cccc} 
    \toprule
      $N$   &  $M$ & Jacobi & Schwarz \\ \midrule 
      $8^3$ & $2^3$ & 33 & 26  \\
      $16^3$ & $4^3$ & 71 & 39  \\
      $32^3$ & $8^3$ & 115 &  53  \\
      $64^3$ & $16^3$ & 206 &  88  \\
    \bottomrule
    \end{tabular}
\end{table}


\cref{t:schwarz_strong_2d,t:schwarz_weak_2d} present results of the Schwarz preconditioner for solving problems in 2D; analogously, \cref{t:schwarz_strong_3d,t:schwarz_weak_3d} present corresponding results in 3D.



% Jacobi 2D
%Table 11, Jacobi: %$512^2$ & $16^2$ & \num{6.95e+00} & \num{1.07e+00} & \num{5.05e-01} & 514 & \num{3.12e+02} \\ 
%
%Jacobi 3D:
%
%M: 64 (4^3)
%$32^3$ & \num{4.16e-01} & \num{6.71e-02} & \num{3.58e-02} & 100 & \num{6.77e+00} \\ 
%
%M: 512 (8^3)
%$64^3$ & \num{2.96e+00} & \num{5.37e-01} & \num{2.82e-01} & 162 & \num{8.50e+01} \\ 
%
%M: 4096 (16^3)
%$128^3$ & \num{1.95e+01} & \num{4.29e+00} & \num{2.41e+00} & 288 & \num{1.17e+03} \\ 
%
%M: 32768 (32^3)
%$256^3$ & \num{1.65e+02} & \num{3.44e+01} & \num{2.85e+01} & 498 & \num{2.96e+04} \\ 


% 2D
%(66^2/34^2)^3/4
%
%512^2:
%
%M=8^2
%$512^2$ & \num{7.57e+01} & \num{4.78e+00} & \num{1.98e+00} & 34 &  7.47e+01 \\ 
%
%M: 256 (16x16)
%$512^2$ & \num{1.25e+01} & \num{1.35e+00} & \num{7.11e-01} & 46 & 3.97e+01 \\ 
%
%M: 1024 (32x32)
%$512^2$ & \num{3.67e+00} & \num{4.24e-01} & \num{3.33e-01} & 70 & 3.08e+01 \\
%
%M: 4096 (64x64)
%$512^2$ & \num{1.75e+00} & \num{1.62e-01} & \num{6.35e-01} & 118 & 8.81e+01 \\ 


\begin{table}
    \centering \small 
    \caption{\em Schwarz preconditioner  in 2D: $N$ fixed.}
    \label{t:schwarz_strong_2d}
    \begin{tabular}{ccccccc} \toprule
        $N$   &  $M$ & $t_f$ & $m_f$ & $t_s$ & $n_{it}$ & $t_{pcg}$  \\ \midrule 
        $512^2$ & $4^2$ & \num{4.98e+02} & \num{1.80e+01} & \num{7.27e+00} & 29 & \num{2.26e+02} \\ 
        $512^2$  & $8^2$ & \num{5.72e+01} & \num{4.78e+00} & \num{2.02e+00} & 34 & \num{8.55e+01} \\ 
        $512^2$ & $16^2$ & \num{8.68e+00} & \num{1.35e+00} & \num{6.59e-01} & 45 & \num{3.81e+01} \\ 
        $512^2$ & $32^2$ & \num{2.83e+00} & \num{4.24e-01} & \num{2.10e-01} & 71 & \num{2.17e+01} \\ 
        $512^2$ & $64^2$ & \num{1.65e+01} & \num{1.62e-01} & \num{2.22e-01} & 116 & \num{4.56e+01} \\ 
    \bottomrule
    \end{tabular}
    \centering \small 
    \caption{\em Schwarz preconditioner in 2D: $N/M$ fixed. $^*$PCG stagnated at relative residuals \num{1.31e-12} and \num{1.47e-12}, respectively.}
    \label{t:schwarz_weak_2d}
    \begin{tabular}{ccccccc} \toprule
        $N$   &  $M$ & $t_f$ & $m_f$ & $t_s$ & $n_{it}$ & $t_{pcg}$  \\ \midrule 
        $512^2$ & $16^2$ & \num{9.53e+00} & \num{1.35e+00} & \num{6.18e-01} & 46 & \num{4.14e+01} \\
        $1024^2$ & $32^2$ & \num{3.53e+01} & \num{5.43e+00} & \num{3.86e+00} & 71 & \num{3.33e+02} \\ 
        $2048^2$ & $64^2$ & \num{1.41e+02} & \num{2.18e+01} & \num{1.81e+01} &$119^*$& \num{2.40e+03} \\ 
        $4096^2$ & $128^2$ & \num{5.63e+02} & \num{8.74e+01} & \num{7.72e+01} &$212^*$& \num{1.89e+04} \\ 
    \bottomrule
    \end{tabular}
\end{table}



% single solve
%
%M = 8^2: 4356
%1.755 s
%M = 16^2: 1156
%0.567 s
%M = 32^2: 324
%0.167 s
%M = 64^2: 100
%0.121 s
%
% single factor, chol takes 1/2 factor time
%N = 65^2: chol=0.517 s, A=0.340 s
%N = 129^2: chol=29.539 s, A=5.287 s



%M: 256 (16x16)
%$512^2$ & \num{1.54e+01} & \num{1.35e+00} & \num{6.99e-01} & 47 & \num{4.34e+01} \\ 
%M: 1024 (32x32)
%$1024^2$ & \num{5.17e+01} & \num{5.43e+00} & \num{3.18e+00} & 71 & \num{2.65e+02} \\ 
%M: 4096 (64x64), 1.00e-12
%$2048^2$ & \num{2.01e+02} & \num{2.18e+01} & \num{1.21e+01} & 119 & \num{1.63e+03} \\ 
%
%
%M: 1024 (32x32)
%$512^2$ & \num{4.16e+00} & \num{4.24e-01} & \num{3.28e-01} & 70 & \num{3.18e+01} \\ 
%M: 4096 (64x64)
%$1024^2$ & \num{1.43e+01} & \num{1.71e+00} & \num{2.68e+00} & 117 & \num{4.38e+02} \\
%M: 16384 (128x128), 1.22e-12
%$2048^2$ & \num{6.19e+01} & \num{6.86e+00} & \num{5.23e+01} & 209 & \num{1.13e+04} \\ 
%M: 65536 (256x256), 2.35e-12
%$4096^2$ & \num{2.30e+02} & \num{2.75e+01} & \num{2.89e+01} & 379 & \num{1.52e+04} \\ 



% 3D
%N=64^3
%M: 64 (4^3)
%$64^3$ & \num{9.57e+01} & \num{7.37e+00} & \num{3.01e+00} & 38 & \num{1.24e+02} \\ 
%M: 512 (8^3)
%$64^3$ & \num{1.04e+01} & \num{1.77e+00} & \num{9.22e-01} & 51 & \num{5.88e+01} \\ 
%M: 4096 (16^3)
%$64^3$ & \num{4.04e+00} & \num{6.80e-01} & \num{8.56e-01} & 87 & \num{9.47e+01} \\ 
%
%nvdimm
%
%M: 8 (2^3)
%$32^3$ & \num{9.67e+00} & \num{7.72e-01} & \num{2.95e-01} & 29 & \num{9.99e+00} \\ 
%M: 64 (4^3)
%$64^3$ & \num{1.12e+02} & \num{7.37e+00} & \num{2.97e+00} & 39 & \num{1.29e+02} \\ 
%M: 512 (8^3)
%$128^3$ & \num{9.52e+02} & \num{6.42e+01} & \num{7.26e+01} & 51 & \num{3.76e+03} \\ 
%M: 4096 (16^3)
%$256^3$ & \num{9.12e+03} & \num{5.35e+02} & \num{4.67e+02} & 83 & \num{4.13e+04} \\ 


%M: 64 (4^3)
%$32^3$ & \num{1.23e+00} & \num{1.90e-01} & \num{9.18e-02} & 39 & \num{4.41e+00} \\ 
%M: 512 (8^3)
%$64^3$ & \num{1.10e+01} & \num{1.77e+00} & \num{9.58e-01} & 52 & \num{6.52e+01} \\ 
%M: 4096 (16^3)
%$128^3$ & \num{9.12e+01} & \num{1.52e+01} & \num{1.51e+01} & 82 & \num{1.43e+03} \\
%M: 32768 (32^3)
%$256^3$ & \num{8.10e+02} & \num{1.26e+02} & \num{1.79e+02} & 156 & \num{3.29e+04} \\

%
% single factor, chol takes 1/2 factor time
%N=9^3: chol=0.005 s, A=0.012 s
%N =17^3: chol=0.778 s, A=0.548 s


\begin{table}
    \centering \small 
    \caption{\em Schwarz preconditioner in 3D: $N$ fixed.}
    \label{t:schwarz_strong_3d}
    \begin{tabular}{ccccccc} \toprule
        $N$   &  $M$ & $t_f$ & $m_f$ & $t_s$ & $n_{it}$ & $t_{pcg}$  \\ \midrule 
        $64^3$ & $2^3$ & \num{2.03e+03} & \num{4.13e+01} & \num{2.61e+01} & 29 & \num{1.27e+03} \\ 
        $64^3$ & $4^3$ & \num{8.43e+01} & \num{7.37e+00} & \num{3.06e+00} & 38 & \num{1.29e+02} \\ 
        $64^3$ & $8^3$ & \num{9.47e+00} & \num{1.77e+00} & \num{8.95e-01} & 51 & \num{5.83e+01} \\ 
        $64^3$ & $16^3$ & \num{3.88e+00} & \num{6.80e-01} & \num{4.57e-01} & 88 & \num{6.25e+01} \\ 
    \bottomrule
    \end{tabular}
    \centering \small 
    \caption{\em Schwarz preconditioner in 3D: $N/M$ fixed.}
    \label{t:schwarz_weak_3d}
    \begin{tabular}{ccccccc} \toprule
        $N$   &  $M$ & $t_f$ & $m_f$ & $t_s$ & $n_{it}$ & $t_{pcg}$  \\ \midrule 
        $32^3$ & $4^3$ & \num{1.03e+00} & \num{1.90e-01} & \num{8.99e-02} & 39 & \num{4.22e+00} \\ 
        $64^3$ & $8^3$ & \num{8.98e+00} & \num{1.77e+00} & \num{8.50e-01} & 52 & \num{5.72e+01} \\ 
        $128^3$ & $16^3$ & \num{7.76e+01} & \num{1.52e+01} & \num{8.79e+00} & 82 & \num{8.84e+02} \\ 
        $256^3$ & $32^3$ & \num{7.48e+02} & \num{1.26e+02} & \num{1.36e+02} & 156 & \num{2.62e+04} \\ 
    \bottomrule
    \end{tabular}
\end{table}



\cref{t:schwarz_strong_2d,t:schwarz_strong_3d} show that when $N$ is fixed, the storage $m_f$ and the application time of the preconditioner $t_s$ scaled approximately as $\bigO(M^{-1})$; see \cref{e:mem}. The factorization time $t_f$ apparently decreased slower than $\bigO(M^{-2})$ as \cref{e:fact} predicts, and that is due to the dominance of the $\bigO(M^{-1})$ cost for evaluating diagonal blocks in $A$ associated with all subdomains. 


\cref{t:schwarz_weak_2d,t:schwarz_weak_3d} show that when $N/M=\bigO(1)$, the factorization time $t_f$, the storage $m_f$ and the application time of the preconditioner $t_s$ all scaled approximately as $\bigO(N)$; see \cref{e:mem}. Assuming the number of PCG iterations $n_{it} = \bigO(M^{1/d})$, we obtain the complexity of the total running time as $\bigO(N^{1+1/d})$. The caveat is that as the problem size increased, the PCG stagnated before reaching the relative residual  $\num{1e-12}$ due to the increasing condition number of matrix $A$ in \cref{e:axb}.


As \cref{t:schwarz_strong_2d,t:schwarz_weak_2d,t:schwarz_strong_3d,t:schwarz_weak_3d} show,  the time spent in the PCG dominated the total running time except for a couple cases where the problem size per subdomain is too large for the preconditioner to be competitive. We had employed the FFT for fast matvec with $A$ in the PCG. In general, the FFT should be replaced by its non-uniform variant or the FMM, both of which have larger pre-factors. As a result, the PCG time is expected to be even more dominant.


As a reference, the Jacobi preconditioner required 514 iterations and \num{3.12e+02} seconds in the PCG for the experiment where $N=512^2$ and $M=16^2$ (compare to the first row in \cref{t:schwarz_weak_2d}). The gap between the Jacobi preconditioner and the Schwarz preconditioner is much smaller for solving problems in 3D. For example,  the Jacobi preconditioner required 162 iterations and \num{8.50e+01} seconds in the PCG for the experiment where $N=64^3$ and $M=8^3$ (compare to the second row in \cref{t:schwarz_weak_3d}).





\begin{figure}
     % 2nd row
     %\centering
     \begin{subfigure}[b]{0.333\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n16}
         \caption{\em $N=16^2, D=M=2^2$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n32}
         \caption{\em $N=32^2, D=M=4^2$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n64}
         \caption{\em $N=64^2, D=M=8^2$}
     \end{subfigure}
     % 1st row
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n16_jacobi}
         \caption{\em $N=16^2, D=M=2^2$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n32_jacobi}
         \caption{\em $N=32^2, D=M=4^2$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n64_jacobi}
         \caption{\em $N=64^2, D=M=8^2$}
     \end{subfigure}
%     % 3rd row
%     \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{eigenvalue_n16_M4}
%         \caption{Schwarz: $N=16^2,M=2^2$}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{eigenvalue_n32_M4}
%         \caption{Schwarz: $N=32^2,M=2^2$}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{eigenvalue_n64_M4}
%         \caption{Schwarz: $N=64^2,M=2^2$}
%     \end{subfigure}     
        \caption{\em Spectrum of preconditioned matrix with  the Schwarz preconditioner (first row) and the block Jacobi  preconditioner (second row), respectively. Recall the matrix and the domain decomposition in \cref{e:a_2d} and \cref{t:dd}, respectively.
        %where a uniform grid in the unit square of size $N$ is partitioned uniformly into $M$ subdomains. 
        }
        \label{f:spectrum}
\end{figure}





\cref{f:spectrum} shows the spectrum of $T^{-1}_\text{Schwarz}A$ and of $T^{-1}_\text{Jacobi}A$ for three experiments. As the figure shows, the eigenvalues of $T^{-1}_\text{Schwarz}A$ are better clustered compared to those of $T^{-1}_\text{Jacobi}A$. In particular, $\lambda_{\min}(T^{-1}_\text{Schwarz}A)$ is almost constant, whereas $\lambda_{\min}(T^{-1}_\text{Jacobi}A)$ decreases toward zero. 




\begin{figure}
     \centering
     \includegraphics[width=0.3\textwidth]{lambda_min}
     \caption{\em The interior, boundary and exterior of $\Omega_k$. Dashed lines are the boundaries of domain partitioning without overlapping. $\Omega_k^b$ is the overlapped region shared by at least two subdomains.}
     \label{f:lambda_min}
\end{figure}

\begin{definition} [Interior, boundary and exterior of a subdomain]
\label{d:subdomain}
Given an overlapping domain decomposition $\{\Omega_1, \Omega_2, \ldots, \Omega_M\}$ of the problem domain $\Omega$, we define the interior, the boundary and the exterior of a subdomain $\Omega_k$ as the following:
\begin{itemize}
\item
$\Omega_k^\mathtt{i} = \Omega / \cup_{i\not=k} \Omega_i$,
\item
$\Omega_k^\mathtt{b} =  \Omega_k / \Omega_k^\mathtt{i}$,
\item
$\Omega_k^\mathtt{e} = \Omega / \Omega_k$.
\end{itemize}
\end{definition}

See \cref{f:lambda_min} for a pictorial illustration of \cref{d:subdomain}. Correspondingly, we can decompose a vector  $x = x_k^\mathtt{i} + x_k^\mathtt{b} + x_k^\mathtt{e}$, where $x_k^\mathtt{i}, x_k^\mathtt{b}$ and $x_k^\mathtt{e}$ are the restriction of $x$ in the interior, the boundary and the exterior of $\Omega_k$, respectively.


\begin{lemma} \label{l:subdomain}
Let $P_j, P_k$ be defined in \cref{e:pi} and $x = x_k^\mathtt{i} + x_k^\mathtt{b} + x_k^\mathtt{e}$. We have the following:
\begin{enumerate}[label={(\arabic*)}]
\item
$P_j x$ is zero in $\Omega_k^\mathtt{i}$ if $j \not=k$;
\item
$P_k x_k^\mathtt{b} = x_k^\mathtt{b}$ and thus  is zero in $\Omega_k^\mathtt{i}$;
\item
$P_k x_k^\mathtt{i} = x_k^\mathtt{i}$.
\end{enumerate}
\end{lemma}
\begin{proof}
It is obvious that (1) holds. We know that solution of an interior Laplace's problem with Dirichlet boundary condition is unique according to potential theory. Therefore, (2) and (3) both hold.
\end{proof}






As \cref{t:js_3d} shows, the minimum eigenvalue of the Schwarz preconditioned matrix increases towards one, which naturally leads to the following conjecture:
\begin{conjecture} %[$\lambda_{\min}(T^{-1} A)=1$ in 3D]
Suppose $A$ is defined in \cref{e:a} as the discretization of the first-kind Fredholm equation for Laplace's equation in 3D and $T^{-1}$ is defined in \cref{e:ad}. Then,
\[
\lambda_{\min}(T^{-1}A) = 1,
\]
as the problem size $N\to\infty$ and the number of subdomains $D=M$ increases proportionally.
\end{conjecture}

Below, we prove that $1$ is an eigenvalue of $T^{-1} A$ (we do not prove 1 is the minimum eigenvalue).


\begin{theorem} %[$\lambda(T^{-1} A)=1$]
%Let $A$ be the discretization of \cref{e:int} in 3D and $T^{-1}$ be defined in \cref{e:ad}. We have
%\[
%\lambda_{\min}(T^{-1}A) = 1.
%\]
Suppose $A$ is defined in \cref{e:a} as the discretization of the first-kind Fredholm equation for Laplace's equation in 3D and $T^{-1}$ is defined in \cref{e:ad}. Then, 1 is an eigenvalue of $T^{-1}A$ as the problem size $N\to\infty$ and the number of subdomains $D=M$ increases proportionally.
\end{theorem}
\begin{proof}
Consider the eigenvalue problem
\[
T^{-1} A x = \sum_{i=1}^D P_i x = \lambda x.
\]
Consider the restriction of both sides to the interior of $\Omega_k$. According to \cref{l:subdomain}, we have
%\[
%P_k (x_k^\mathtt{i} + x_k^\mathtt{e}) = R_k^\top A_k^{-1} R_k A (x_k^\mathtt{i} + x_k^\mathtt{e}) = \lambda x_k^\mathtt{i},
%\]
%and also
\begin{equation} \label{e:min}
P_k  x_k^\mathtt{e} = R_k^\top A_k^{-1} R_k A x_k^\mathtt{e} = (\lambda - 1) x_k^\mathtt{i},
\end{equation}
%\red{TODO: multiply by $(x_k^\mathtt{i})^\top A$ or $(x_k^\mathtt{e})^\top A$}

As the problem size $N\to\infty$ and the number of subdomains $D=M$ increases proportionally, we know from potential theory that the harmonic field $A x_k^\mathtt{e}$ on $\Omega_k$ caused by $x_k^\mathtt{e}$ outside of $\Omega_k$ can be exactly replicated by a source distribution on $\Omega_k^\mathtt{b}$\footnote{The electrostatic shielding effect in physics.}. Therefore, the right hand side of \cref{e:min} is zero, and thus $\lambda=1$.
\end{proof}


==> tmp.tex <==


\begin{figure}
     % 2nd row
     %\centering
     \begin{subfigure}[b]{0.333\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n16}
         \caption{\em $N=16^2, D=M=2^2$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n32}
         \caption{\em $N=32^2, D=M=4^2$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n64}
         \caption{\em $N=64^2, D=M=8^2$}
     \end{subfigure}
     % 1st row
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n16_jacobi}
         \caption{\em $N=16^2, D=M=2^2$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n32_jacobi}
         \caption{\em $N=32^2, D=M=4^2$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{eigenvalue_n64_jacobi}
         \caption{\em $N=64^2, D=M=8^2$}
     \end{subfigure}
%     % 3rd row
%     \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{eigenvalue_n16_M4}
%         \caption{Schwarz: $N=16^2,M=2^2$}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{eigenvalue_n32_M4}
%         \caption{Schwarz: $N=32^2,M=2^2$}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{eigenvalue_n64_M4}
%         \caption{Schwarz: $N=64^2,M=2^2$}
%     \end{subfigure}     
        \caption{\em Spectrum of preconditioned matrix with  the Schwarz preconditioner (first row) and the block Jacobi  preconditioner (second row), respectively. Recall the matrix and the domain decomposition in \cref{e:a_2d} and \cref{t:dd}, respectively.
        %where a uniform grid in the unit square of size $N$ is partitioned uniformly into $M$ subdomains. 
        }
        \label{f:spectrum}
\end{figure}





\cref{f:spectrum} shows the spectrum of $T^{-1}_\text{Schwarz}A$ and of $T^{-1}_\text{Jacobi}A$ for three experiments. As the figure shows, the eigenvalues of $T^{-1}_\text{Schwarz}A$ are better clustered compared to those of $T^{-1}_\text{Jacobi}A$. In particular, $\lambda_{\min}(T^{-1}_\text{Schwarz}A)$ is almost constant, whereas $\lambda_{\min}(T^{-1}_\text{Jacobi}A)$ decreases toward zero. 




\begin{figure}
     \centering
     \includegraphics[width=0.3\textwidth]{lambda_min}
     \caption{\em The interior, boundary and exterior of $\Omega_k$. Dashed lines are the boundaries of domain partitioning without overlapping. $\Omega_k^b$ is the overlapped region shared by at least two subdomains.}
     \label{f:lambda_min}
\end{figure}

\begin{definition} [Interior, boundary and exterior of a subdomain]
\label{d:subdomain}
Given an overlapping domain decomposition $\{\Omega_1, \Omega_2, \ldots, \Omega_M\}$ of the problem domain $\Omega$, we define the interior, the boundary and the exterior of a subdomain $\Omega_k$ as the following:
\begin{itemize}
\item
$\Omega_k^\mathtt{i} = \Omega / \cup_{i\not=k} \Omega_i$,
\item
$\Omega_k^\mathtt{b} =  \Omega_k / \Omega_k^\mathtt{i}$,
\item
$\Omega_k^\mathtt{e} = \Omega / \Omega_k$.
\end{itemize}
\end{definition}

See \cref{f:lambda_min} for a pictorial illustration of \cref{d:subdomain}. Correspondingly, we can decompose a vector  $x = x_k^\mathtt{i} + x_k^\mathtt{b} + x_k^\mathtt{e}$, where $x_k^\mathtt{i}, x_k^\mathtt{b}$ and $x_k^\mathtt{e}$ are the restriction of $x$ in the interior, the boundary and the exterior of $\Omega_k$, respectively.


\begin{lemma} \label{l:subdomain2}
Let $P_j, P_k$ be defined in \cref{e:pi} and $x = x_k^\mathtt{i} + x_k^\mathtt{b} + x_k^\mathtt{e}$. We have the following:
\begin{enumerate}[label={(\arabic*)}]
\item
$P_j x$ is zero in $\Omega_k^\mathtt{i}$ if $j \not=k$;
\item
$P_k x_k^\mathtt{b} = x_k^\mathtt{b}$ and thus  is zero in $\Omega_k^\mathtt{i}$;
\item
$P_k x_k^\mathtt{i} = x_k^\mathtt{i}$.
\end{enumerate}
\end{lemma}
\begin{proof}
It is obvious that (1) holds. We know that solution of an interior Laplace's problem with Dirichlet boundary condition is unique according to potential theory. Therefore, (2) and (3) both hold.
\end{proof}






As \cref{t:js_3d} shows, the minimum eigenvalue of the Schwarz preconditioned matrix increases towards one, which naturally leads to the following conjecture:
\begin{conjecture} %[$\lambda_{\min}(T^{-1} A)=1$ in 3D]
Suppose $A$ is defined in \cref{e:a} as the discretization of the first-kind Fredholm equation for Laplace's equation in 3D and $T^{-1}$ is defined in \cref{e:ad}. Then,
\[
\lambda_{\min}(T^{-1}A) = 1,
\]
as the problem size $N\to\infty$ and the number of subdomains $D=M$ increases proportionally.
\end{conjecture}

Below, we prove that $1$ is an eigenvalue of $T^{-1} A$ (we do not prove 1 is the minimum eigenvalue).


\begin{theorem} %[$\lambda(T^{-1} A)=1$]
%Let $A$ be the discretization of \cref{e:int} in 3D and $T^{-1}$ be defined in \cref{e:ad}. We have
%\[
%\lambda_{\min}(T^{-1}A) = 1.
%\]
Suppose $A$ is defined in \cref{e:a} as the discretization of the first-kind Fredholm equation for Laplace's equation in 3D and $T^{-1}$ is defined in \cref{e:ad}. Then, 1 is an eigenvalue of $T^{-1}A$ as the problem size $N\to\infty$ and the number of subdomains $D=M$ increases proportionally.
\end{theorem}
\begin{proof}
Consider the eigenvalue problem
\[
T^{-1} A x = \sum_{i=1}^D P_i x = \lambda x.
\]
Consider the restriction of both sides to the interior of $\Omega_k$. According to \cref{l:subdomain2}, we have
%\[
%P_k (x_k^\mathtt{i} + x_k^\mathtt{e}) = R_k^\top A_k^{-1} R_k A (x_k^\mathtt{i} + x_k^\mathtt{e}) = \lambda x_k^\mathtt{i},
%\]
%and also
\begin{equation} \label{e:min}
P_k  x_k^\mathtt{e} = R_k^\top A_k^{-1} R_k A x_k^\mathtt{e} = (\lambda - 1) x_k^\mathtt{i},
\end{equation}
%\red{TODO: multiply by $(x_k^\mathtt{i})^\top A$ or $(x_k^\mathtt{e})^\top A$}

As the problem size $N\to\infty$ and the number of subdomains $D=M$ increases proportionally, we know from potential theory that the harmonic field $A x_k^\mathtt{e}$ on $\Omega_k$ caused by $x_k^\mathtt{e}$ outside of $\Omega_k$ can be exactly replicated by a source distribution on $\Omega_k^\mathtt{b}$\footnote{The electrostatic shielding effect in physics.}. Therefore, the right hand side of \cref{e:min} is zero, and thus $\lambda=1$.
\end{proof}
